Separability and complete reducibility of subgroups of the Weyl group of a simple algebraic group of type $E_7$

Let $G$ be a connected reductive algebraic group defined over an algebraically closed field $k$. The aim of this paper is to present a method to find triples $(G,M,H)$ with the following three properties. Property 1: $G$ is simple and $k$ has characteristic 2. Property 2: $H$ and $M$ are closed reductive subgroups of $G$ such that $H<M<G$, and $(G,M)$ is a reductive pair. Property 3: $H$ is $G$-completely reducible, but not $M$-completely reducible. We exhibit our method by presenting a new example of such a triple in $G=E_7$. Then we consider a rationality problem and a problem concerning conjugacy classes as important applications of our construction.

==> G2-example.tex <==
\section{The $G_2$ example}
\begin{ass}
For the rest of the paper, we assume $p=2$.
\end{ass}
We recall the $G_2$ example~\cite[Sec.~7]{Ben1} to exhibit our method to find a triple (G, M, H) with the desired property. Our approach to the $G_2$ example is different from~\cite[Sec.~7]{Ben1} in the following sense. 
\begin{enumerate}
\item We show the importance of a non-separable action of $K$ on $R_u(P)$.
\item We explain how to choose $v$ to get $H=v K v^{-1}$. 
\item We use Proposition~\ref{GIT}; see Remark~\ref{reason}.
\end{enumerate}

\subsection{Step 1}
Let $G$ be a simple algebraic group of type $G_2$ defined over $k$ of characteristic $2$. Fix a maximal torus $T$ of $G$ and a Borel subgroup $B$ of $G$ containing $T$. Then we have $\Psi^{+}(G) = \{\alpha, \beta, \alpha+\beta, 2\alpha+\beta, 3\alpha+\beta, 3\alpha+2\beta\}$ where $\alpha$ is short and $\beta$ is long~\cite[Sec.~33.5]{Humphreys}. We call the roots whose coefficient of $\beta$ is $2$ \emph{weight-2} roots, and the roots whose coefficient of $\beta$ is $1$ \emph{weight-1} roots respectively. 
Define 
\begin{alignat*}{2}
L_\alpha :&= \langle T, G_\alpha \rangle, \\
P_\alpha :&= \langle L_\alpha, U_\beta, U_{\alpha+\beta}, U_ {2\alpha+\beta}, U_{3\alpha+\beta}, U_{3\alpha+2\beta} \rangle. 
\end{alignat*}
Then $P_\alpha$ is a parabolic subgroup of $G$, and $L_\alpha$ is a Levi subgroup of $P_\alpha$. We have 
\begin{equation*}
\Psi(R_u(P_\alpha))=\{ \beta, \alpha+\beta, 2\alpha+\beta, 3\alpha+\beta, 3\alpha+2\beta\}.
\end{equation*}
Pick $\alpha^{\vee}(t)\in \alpha^{\vee}(k^{*})$ of order $3$, and define
\begin{equation*}
K := \langle n_\alpha, \alpha^{\vee}(t) \rangle.
\end{equation*}
From~\cite[Sec.~7]{Ben1}, we obtain the orbits of $\langle n_\alpha \rangle$ on $\Psi(R_u(P_\alpha))$. 
\begin{equation}\label{Orbits in G-2}
O_1=\{\beta, 3\alpha+\beta\},\; O_2=\{\alpha+\beta, 2\alpha+\beta\},\; O_3=\{3\alpha+2\beta\}. 
\end{equation}
By~\cite[Sec.~7]{Ben1}
\begin{alignat}{2}
&\alpha^{\vee}(t) \textup{ acts trivially on } U_\beta, U_ {3\alpha+\beta}, U_{3\alpha+2\beta}, \mathfrak{u}_\beta, \mathfrak{u}_ {3\alpha+\beta}, \mathfrak{u}_{3\alpha+2\beta}. \nonumber\\
&\alpha^{\vee}(t) \textup{ acts non-trivially on } U_{\alpha+\beta}, U_ {2\alpha+\beta}, \label{action of T} \mathfrak{u}_{\alpha+\beta}, \mathfrak{u}_ {2\alpha+\beta}. 
\end{alignat}
Since $K$ is generated by $n_\alpha$ and $\alpha^{\vee}(t)$, a slight variant of Proposition~\ref{infinitesimal centralizer lemma} with (\ref{Orbits in G-2}) and (\ref{action of T}) yields

\begin{prop}\label{inf-G_2}
$\mathfrak{c}_{\textup{Lie}\,(R_u(P_\alpha))}(K) = \{a(e_\beta + e_{3\alpha+\beta}) + b(e_{3\alpha+2\beta}) \mid a, b\in k\}$.
\end{prop}

The next result is crucial for our argument. 
\begin{prop}\label{glo-G_2}
$C_{R_u(P_\alpha)}(K) = U_{3\alpha+2\beta}$.
\end{prop}

\begin{proof}
Let $u\in C_{R_u(P_\alpha)}(K)$. By Lemma~\ref{unipotent radical lemma}, $u$ can be expressed uniquely as
\begin{alignat*}{2}
u &= \epsilon_{\beta}(a_\beta) \epsilon_{3\alpha+\beta}(a_{3\alpha+\beta}) \epsilon_{\alpha+\beta}(a_{\alpha+\beta}) \epsilon_{2\alpha+\beta}(a_{2\alpha+\beta}) \epsilon_{3\alpha+2\beta}(a_{3\alpha+2\beta}), \\
&\textup{ for some } a_\beta, a_{3\alpha+\beta}, a_{\alpha+\beta}, a_{2\alpha+\beta}, a_{3\alpha+2\beta} \in k. 
\end{alignat*} 
Since $\alpha^{\vee}(t)$ must act trivially on $U_{\alpha+\beta}$ and $U_ {2\alpha+\beta}$, (\ref{action of T}) yields
\begin{equation*}
a_{\alpha+\beta}=a_{2\alpha+\beta}=0.
\end{equation*}
From \cite[Sec.~7]{Ben1}, we obtain
\begin{equation*}
n_\alpha u n_\alpha^{-1} = \epsilon_\beta(a_{3\alpha+\beta})\epsilon_{3\alpha+\beta}(a_\beta)\epsilon_{3\alpha+2\beta}(a_\beta a_{3\alpha+\beta}+a_{3\alpha+2\beta}).
\end{equation*}
Since $u$ is centralized by $n_\alpha$, we have 
\begin{equation*}
a_\beta=a_{3\alpha+\beta}, a_\beta a_{3\alpha+\beta}=0. 
\end{equation*}
Thus we have 
\begin{equation*}
a_\beta=a_{3\alpha+\beta}=0.
\end{equation*}
\end{proof}
\begin{prop}\label{1-D non-sep}
$K$ acts non-separably on $R_u(P_\alpha)$.
\end{prop} 
\begin{proof}
This follows from Proposition~\ref{inf-G_2} and \ref{glo-G_2}.
\end{proof}
\subsection{Step 2}
Let 
\begin{equation*}
C:=\{\epsilon_{\beta}(a)\epsilon_{3\alpha+\beta}(a)\mid a\in k\}.
\end{equation*} 
\begin{rem}
The 1-dimensional curve $C$ was chosen so that $T_1(C)$ is tangent to $\mathfrak{c}_{\text{Lie}\,(R_u(P_\alpha))}(K)$ but not tangent to $\text{Lie}\,C_{R_u(P_\alpha)}(K)$. 
\end{rem}
\noindent Pick any $a\in k^{*}$. Let $v(a)\in C$. We have
\begin{alignat}{2}
v(a) n_\alpha v(a)^{-1} &= n_\alpha \epsilon_{3\alpha+2\beta}(a^2), \label{star}\\
v(a) \alpha^{\vee}(t) v(a)^{-1} &= \alpha^{\vee}(t). \nonumber 
\end{alignat} 
Now set
\begin{alignat*}{2}
H = v(a) K v(a)^{-1} & = \langle n_\alpha \epsilon_{3\alpha+2\beta}(a^2), \alpha^{\vee}(t) \rangle, \\
M & = \langle L_\alpha, G_{3\alpha+2\beta} \rangle. 
\end{alignat*}
\begin{rem}\label{G2M}
$M$ was chosen so that $M$ is generated by a Levi subgroup $L_\alpha$ containing $H$ and all root subgroups of even $\beta$-weight where $\beta$ is the simple root not contained in $\Psi(L_\alpha)$. It is easy to see that $(G,M)$ is a reductive pair since $\Psi(M,T)$ is a closed subsystem of $\Psi(G,T)$, \cite[Lem.~3.9]{Ben1}.
\end{rem}
\noindent Then we have 
\begin{equation*}
H\subset M, \,
H\not\subset L_\alpha. 
\end{equation*}
\begin{prop}
$H$ is not $M$-cr.
\end{prop}
\begin{proof} 
First, let 
\begin{equation*}
\lambda = \alpha^{\vee} + 2\beta^{\vee}. 
\end{equation*}
Since we have $\langle \alpha, \lambda \rangle = 0$ and $\langle \beta, \lambda \rangle = 1$, it is easy to see that
\begin{equation*}
L_\alpha = L_\lambda, \, P_{\alpha} = P_\lambda. 
\end{equation*}
Let $c_\lambda: P_\lambda\rightarrow L_\lambda$ be the homomorphism from Definition~\ref{homomorphism}. Suppose that $H$ is $M$-cr. By Proposition \ref{GIT}, it is enough to show that there is an element $h\in H$ which is not $R_u(P_\lambda(M))$-conjugate to $c_\lambda(h)$. Set
\begin{equation*}\label{form of h}
h:= v(a) n_\alpha v(a)^{-1}=n_\alpha \epsilon_{3\alpha+2\beta}(a^2).
\end{equation*}
Then we have 
\begin{alignat*}{2}
c_\lambda(h) &= \lim_{x\rightarrow 0}\left(\lambda(x)v(a) n_\alpha v(a)^{-1}\lambda(x)^{-1}\right)\\
                     &= \lim_{x\rightarrow 0}\left(\lambda(x)n_\alpha \epsilon_{3\alpha+2\beta}(a^2)\lambda(x)^{-1}\right)\\
                     &= n_\alpha. 
\end{alignat*}
\noindent Now suppose that $h$ is $R_u(P_\lambda(M))$-conjugate to $c_\lambda(h)=n_\alpha$. Then there exists $m\in R_u(P_\lambda(M))$ such that
\begin{equation*}
m v(a)n_\alpha v(a)^{-1} m^{-1}=n_\alpha. 
\end{equation*}
Since $m\in U_{3\alpha+2\beta}$ centralizes $n_\alpha$ and $v(a)$, this implies
\begin{equation*}
v(a) n_\alpha v(a)^{-1}=n_\alpha. 
\end{equation*}
This contradicts (\ref{star}).
\end{proof}

\begin{rem}\label{reason}
In \cite[Sec.~7, Prop~.7.17]{Ben1}, Bate et al.~used  \cite[Lem.~2.17 and Thm.~3.1]{Ben2} to turn a problem on $M$-complete reducibility into a problem involving $M$-conjugacy. We have used Proposition~\ref{GIT} to turn the same problem into a problem involving $R_u(P\cap M)$-conjugacy, which is easier.
\end{rem}
 
\subsection{Step~3}
\begin{prop}
$H$ is $G$-cr. 
\end{prop}
\begin{proof}
See \cite[Lem.~7.10(a)]{Ben1}.
\end{proof}  
